Analysis-aware defeaturing of complex geometries with Neumann features

Local modifications of a computational domain are often performed in order to simplify the meshing process and to reduce computational costs and memory requirements. However, removing geometrical features of a domain often introduces a non-negligible error in the solution of a differential problem in which it is defined. In this work, we extend the results from [1] by studying the case of domains containing an arbitrary number of distinct Neumann features, and by performing an analysis on Poisson's, linear elasticity, and Stokes' equations. We introduce a simple, computationally cheap, reliable, and efficient a posteriori estimator of the geometrical defeaturing error. Moreover, we also introduce a geometric refinement strategy that accounts for the defeaturing error: Starting from a fully defeatured geometry, the algorithm determines at each iteration step which features need to be added to the geometrical model to reduce the defeaturing error. These important features are then added to the (partially) defeatured geometrical model at the next iteration, until the solution attains a prescribed accuracy. A wide range of two- and three-dimensional numerical experiments are finally reported to illustrate this work.

==> linelast.tex <==
In this section, we consider a linear elasticity problem, and, following the same structure as for the Poisson's problem in Section~\ref{s:poisson}, we precisely define the exact $\mathcal P(\Omega)$, defeatured $\mathcal P(\Omega_0)$, and extension problems $\mathcal P\big(\tilde F_\mathrm p^k\big)$ for all $k=1,\ldots,N_f$. Then in this context, we give a precise definition of the proposed reliable and efficient \textit{a posteriori} estimator $\mathscr E(\boldsymbol u_\mathrm d)$ of the energy norm of the defeaturing error $\vertiii{\boldsymbol u-\boldsymbol u_\mathrm d}_\Omega$.

In the following, we denote by $\boldsymbol H^s(D):= \left[ H^s(D) \right]^n$ the vector-valued Sobolev space of order $s\in\mathbb R$ in a domain $D\subset \mathbb R^n$, whose classical norm and semi-norm are again written $\|\cdot\|_{s,D}$ and $|\cdot|_{s,D}$, respectively. We will also denote by $\boldsymbol L^2(D):=\boldsymbol H^0(D)$. Moreover, if we let $\varphi \subset \partial D$ and $\boldsymbol z\in \boldsymbol H^\frac{1}{2}(\varphi)$, and to be able to deal with boundary conditions, we will denote by
$$\boldsymbol H_{\boldsymbol z,\varphi}^1(D) := \{ \boldsymbol y\in \boldsymbol H^1(D): \mathrm{tr}_\varphi(\boldsymbol y)=\boldsymbol z\},$$
where $\mathrm{tr}_\varphi(\boldsymbol y)$ denotes the trace of $\boldsymbol y$ on $\varphi$.
%For every scalar-valued functional space presented in this chapter, the corresponding space of vector-valued functions of dimension n is denoted in bold, and the corresponding space of tensor-valued functions of dimension n×n is denoted in blackboard bold. That is, for instance, we denote by Lp(D) := [Lp(D)]n and Lp(D) := [Lp(D)]n×n for all p ∈ [1, ∞], and the corresponding norms are computed component-wise. 

\subsection{Exact and defeatured problems}
Let us first introduce the linear elasticity problem $\mathcal P(\Omega)$ in the exact geometry $\Omega$. To do so, considering a function $\boldsymbol v:\Omega\to\mathbb R^n$, let
\begin{equation} \label{eq:linearizestrain}
	\tensorepsilon(\boldsymbol v) := \displaystyle\frac{1}{2} \left(\boldsymbol\nabla \boldsymbol v + \boldsymbol\nabla \boldsymbol v^\top\right)
\end{equation}
be the linearized strain rate tensor, and let $\tensorsigma(\boldsymbol v)$ be the Cauchy stress tensor in the medium.
Then the linear elastic regime is governed by the constitutive relation called Hooke's law which is defined by
\begin{equation} \label{eq:constitutiverelation}
	\tensorsigma(\boldsymbol v) = 2\mu\,\tensorepsilon(\boldsymbol v) + \lambda (\boldsymbol \nabla \cdot \boldsymbol v)\pmb{\mathbb I}_n,
\end{equation}
where $\lambda$ and $\mu$ denote the first and second Lam\'e coefficients, respectively, and $\pmb{\mathbb I}_n$ is the identity tensor in $\mathbb R^{n\times n}$. Owing to thermodynamic stability, we know that $\mu>0$ and $\lambda + \displaystyle \frac 23 \mu > 0$ a.e.\ in $\Omega$. Therefore, we assume that there exist $\mu_\text{min}, \kappa_\text{min} > 0$ such that
\begin{equation} \label{eq:assumptionslame}
	\mu, \lambda \in L^\infty(\Omega), \quad \mu(x) \geq \mu_\text{min}, \quad \lambda(x)+\frac{2}{3}\mu(x) \geq \kappa_\text{min}, \quad \text{ a.e. in } \Omega.
\end{equation}
\begin{assumption} \label{asid:lame_constant}
	Hereinafter, for the sake of simplicity in the exposition, we assume that the Lam\'e constants $\lambda$ and $\mu$ are constant everywhere, and therefore are naturally extended to defeatured geometry $\Omega_0$.
\end{assumption}

Now, let $\boldsymbol g_D\in \boldsymbol H^{\frac{3}{2}}(\Gamma_D)$, $\boldsymbol g\in \boldsymbol H^{\frac{1}{2}}(\Gamma_N)$, and $\boldsymbol f\in \boldsymbol L^2\left(\Omega\right)$. We are interested in the following linear elasticity problem defined in the exact geometry $\Omega$: find $\boldsymbol u:\boldsymbol H^{1}(\Omega)$, the weak solution of
\begin{align}
	\mathcal P(\Omega): \quad
	\begin{cases}
		-\boldsymbol \nabla \cdot \tensorsigma(\boldsymbol u) =\boldsymbol f & \text{ in } \Omega    \\
		\boldsymbol u = \boldsymbol g_D                                      & \text{ on } \Gamma_D  \\
		\tensorsigma(\boldsymbol u)\mathbf{n} = \boldsymbol g                & \text{ on } \Gamma_N,
	\end{cases}\label{eqid:originalpblinelast}
\end{align}
that is, $\boldsymbol u \in \boldsymbol H^1_{\boldsymbol g_D, \Gamma_D}(\Omega)$ satisfies for all $ \boldsymbol v\in \boldsymbol H^1_{\boldsymbol 0,\Gamma_D}(\Omega)$,
\begin{align}
	 & \mathfrak a(\boldsymbol u,\boldsymbol v) := \int_\Omega \tensorsigma(\boldsymbol u) : \tensorepsilon(\boldsymbol v) \,\mathrm dx = \int_\Omega \boldsymbol f \cdot \boldsymbol v \,\mathrm dx + \int_{\Gamma_N} \boldsymbol g \cdot \boldsymbol v \,\mathrm ds. % =: \mathfrak{f}(\boldsymbol v).
	\label{eqid:weakoriginalpblinelast}
\end{align}
If we equip $\boldsymbol H^1_{\boldsymbol 0, \Gamma_D}(\Omega)$ with the norm $\| \boldsymbol \nabla \boldsymbol\cdot \|_{0,\Omega}$, it can be shown that under the assumptions written in~\eqref{eq:assumptionslame} on the Lam\'e coefficients, by Lax-Milgram theorem, problem~\eqref{eqid:weakoriginalpblinelast} is well-posed. However, note that this problem is rarely solved in practice, as it is assumed to be computationally too expensive.


Let us therefore introduce the corresponding linear elasticity problem $\mathcal P(\Omega_0)$ in the defeatured geometry $\Omega_0$. To do so, we need to consider an $\boldsymbol L^2$-extension of the restriction $\boldsymbol f\vert_{\Omega_\star}$ in all the negative components $F_\mathrm n^k$, $k=1,\ldots,N_f$, that we still write $\boldsymbol f\in \boldsymbol L^2(\Omega_0)$ by abuse of notation. Moreover, we assume that the constitutive relation~\eqref{eq:constitutiverelation} governing the linear elastic regime of the body deformation is also valid on functions defined everywhere in $\Omega_0$, with the Lam\'e coefficients also satisfying~\eqref{eq:assumptionslame} in the negative components of the features. Then, instead of~\eqref{eqid:originalpblinelast}, we solve the following defeatured linear elasticity problem: after choosing $\boldsymbol g_0\in \boldsymbol H^{\frac{1}{2}}\left(\gamma_0\right)$, find the weak solution $\boldsymbol u_0\in \boldsymbol H^1(\Omega_0)$ of
\begin{align} \label{eqid:simplpblinelast}
	\mathcal P(\Omega_0): \quad \begin{cases}
		-\boldsymbol \nabla \cdot \tensorsigma(\boldsymbol u_0) =\boldsymbol f & \text{ in } \Omega_0                 \\
		\boldsymbol u_0 = \boldsymbol g_D                                      & \text{ on } \Gamma_D                 \\
		\tensorsigma(\boldsymbol u_0)\mathbf{n} = \boldsymbol g                & \text{ on } \Gamma_N\setminus \gamma \\
		\tensorsigma(\boldsymbol u_0)\mathbf{n}_0 = \boldsymbol g_0            & \text{ on } \gamma_0,
	\end{cases}
\end{align}
that is, $\boldsymbol u_0\in \boldsymbol H^1_{\boldsymbol g_D,\Gamma_D}(\Omega_0)$ satisfies for all $\boldsymbol v_0\in \boldsymbol H^1_{\boldsymbol 0,\Gamma_D}(\Omega_0)$,
\begin{equation} \label{eq:weaksimplpb0linelast}
	\int_{\Omega_0} \tensorsigma(\boldsymbol u_0) : \tensorepsilon(\boldsymbol v_0) \,\mathrm dx = \int_{\Omega_0} \boldsymbol f \cdot \boldsymbol v_0 \,\mathrm dx + \int_{\Gamma_N\setminus \gamma} \boldsymbol g \cdot \boldsymbol v_0 \,\mathrm ds + \int_{\gamma_0} \boldsymbol g_0 \cdot \boldsymbol v_0 \,\mathrm ds.
\end{equation}
From Lax-Milgram theorem, we know that problem~\eqref{eq:weaksimplpb0linelast} is well-posed. Analogously to Poisson's problem, the choice of the defeatured problem data $\boldsymbol f$ in $F_\mathrm n^k$ for $k=1,\ldots,N_f$ and $\boldsymbol g_0$ on $\gamma_0$ will be guided by Remark~\ref{rmk:compatcondmultilinelast}. We only anticipate here that, as before, the best possible choices allow for the conservation of the solution flux in the positive and negative components of the features. That is, the best possible choices verify for all $k=1,\ldots,N_f$,
\begin{align}
	\int_{\gamma_{0,\mathrm p}^{k}} \boldsymbol g_{0} \,\mathrm ds = \int_{\gamma_\mathrm p^k} \boldsymbol g \,\mathrm{d}s + \int_{F_\mathrm p^k} \boldsymbol f\,\mathrm dx \qquad
	\text{ and } \qquad \int_{\gamma_{0,\mathrm n}^{k}} \boldsymbol g_{0} \,\mathrm ds = \int_{\gamma_\mathrm n^{k}} \boldsymbol g \,\mathrm{d}s - \int_{F_\mathrm n^k} \boldsymbol f\,\mathrm dx. \label{eq:compatcondmultilinelast}
\end{align}

Now, for all $k=1,\ldots,N_f$, we need to extend the solution $\boldsymbol u_0$ of~\eqref{eq:weaksimplpb0linelast} to $\tilde F^k_\mathrm p$ as discussed in Section~\ref{ss:pbpres}, where $\tilde F^k_\mathrm p$ satisfies the properties given in~\eqref{eq:condextension}. To do so, let us choose an $\boldsymbol L^2$-extension of the restriction $\boldsymbol f\vert_{F_\mathrm p^k}$ in $G_\mathrm p^k :=\tilde F_\mathrm p^k \setminus \overline{F_\mathrm p^k}$, that we still write $\boldsymbol f$ by abuse of notation, and let us assume that the constitutive relation~\eqref{eq:constitutiverelation} governing the linear elastic regime of the body deformation is also valid for functions defined in $\tilde F_\mathrm p^k$, with the Lam\'e coefficients satisfying~\eqref{eq:assumptionslame}.
Then, similarly to~\eqref{eqid:featurepbmulti}, we define for all $k=1,\ldots,N_f$ the following extension of the solution $\boldsymbol u_0$ of~\eqref{eqid:simplpblinelast} in $\tilde F^k_\mathrm p$, for $k=1,\ldots,N_f$: after choosing $\tilde{\boldsymbol g}^k\in \boldsymbol H^\frac{1}{2}(\tilde \gamma^k)$, find $\boldsymbol u_k\in \boldsymbol H^1\left(\tilde F_\mathrm p^k\right)$, the weak solution of
\begin{align} \label{eq:featurepblinelast}
	\mathcal P\Big(\tilde F_\mathrm p^k\Big): \quad \begin{cases}
		-\boldsymbol \nabla \cdot \tensorsigma(\boldsymbol u_k) =\boldsymbol f      & \text{ in } \tilde{F}_\mathrm p^k  \\
		\boldsymbol u_k = \boldsymbol u_0                                           & \text{ on } \gamma_{0,\mathrm p}^k \\
		\tensorsigma(\boldsymbol u_k)\tilde{\mathbf{n}}^k = \tilde{\boldsymbol g}^k & \text{ on } \tilde \gamma^k        \\
		\tensorsigma(\boldsymbol u_k)\tilde{\mathbf{n}}^k = \boldsymbol g           & \text{ on } \gamma_\intersign^k,
	\end{cases}
\end{align}
that is, $\boldsymbol u_k\in \boldsymbol H^1_{\boldsymbol u_0,\gamma_{0,\mathrm p}^k}\left(\tilde F_\mathrm p^k\right)$ satisfies for all $\boldsymbol v^k\in \boldsymbol H^1_{\boldsymbol 0,\gamma_{0,\mathrm p}^k}\left(\tilde{F}_\mathrm p^k\right)$,
\begin{equation} \label{eq:weakfeaturepblinelast}
	\int_{\tilde{F}_\mathrm p^k} \tensorsigma(\boldsymbol u_k) : \tensorepsilon(\boldsymbol v^k) \,\mathrm dx = \int_{\tilde{F}_\mathrm p^k} \boldsymbol f \cdot \boldsymbol v^k \,\mathrm dx + \int_{\tilde \gamma^k} \tilde{\boldsymbol g}^k \cdot \boldsymbol v^k \,\mathrm ds + \int_{\gamma_\intersign^k} \boldsymbol g \cdot \boldsymbol v^k \,\mathrm ds.
\end{equation}
From Lax-Milgram theorem, we know that problem~\eqref{eq:weakfeaturepblinelast} is well-posed. The choice of the defeatured problem data $\boldsymbol f$ in $G_\mathrm p^k$, and $\tilde{\boldsymbol g}^k$ on $\tilde \gamma^k$ for $k=1,\ldots,N_f$ will be guided as well by Remark~\ref{rmk:compatcondmultilinelast}. As before, the best possible choices allow for the conservation of the solution flux in every feature extension $G_\mathrm p^k$. I.e., they verify for all $k=1,\ldots,N_f$,
\begin{align}
	\int_{\tilde \gamma^k} \tilde{\boldsymbol g}^k \,\mathrm ds = \int_{\gamma^k_{\setminussign}} \boldsymbol g \,\mathrm{d}s - \int_{\tilde F_\mathrm p^k\setminus F_\mathrm p^k} \boldsymbol f\,\mathrm dx. \label{eq:compatcondmultilinelast2}
\end{align}

Then, the defeatured solution $\boldsymbol u_\mathrm d\in \boldsymbol H_{\boldsymbol g_D,\Gamma_D}(\Omega)$ is defined from $\boldsymbol u_0$, and $\boldsymbol u_k$ for $k=1,\ldots,N_f$ as in~\eqref{eqid:defudmulti} and the energy norm of the defeaturing error is defined as
\begin{equation}\label{eq:defeaterrorlinelast}
	\vertiii{\boldsymbol u-\boldsymbol u_\mathrm d}_\Omega := \big(\mathfrak a(\boldsymbol u - \boldsymbol u_\mathrm d, \boldsymbol u - \boldsymbol u_\mathrm d)\big)^\frac{1}{2} = \left(\int_\Omega \tensorsigma(\boldsymbol u-\boldsymbol u_\mathrm d) : \tensorepsilon(\boldsymbol u-\boldsymbol u_\mathrm d) \,\mathrm dx\right)^\frac{1}{2}.
\end{equation}


\subsection{Defeaturing error estimator}
Let us recall the definition of the defeatured solution $\boldsymbol u_\mathrm d$ from~\eqref{eqid:defudmulti}, and the definitions of $\Sigma$, $\Sigma^k$, $\Sigma_\mathrm n$, $\Sigma_{0,\mathrm p}$ and $\Sigma_\setminussign$ from~\eqref{eq:sigmamulti}. Then for all $\boundarypiece \in \Sigma$, let $k_\boundarypiece \equiv k$ if $\boundarypiece \in \Sigma^k$ for some $k=1,\ldots,N_f$, and let
\begin{equation} \label{eqmfel:dsigma}
	\boldsymbol d_\boundarypiece \equiv \begin{cases}\vspace{1mm}
		\boldsymbol g - \tensorsigma(\boldsymbol u_\mathrm d)\mathbf{n}                                     & \text{if } \boundarypiece \in \Sigma_\mathrm n \text{ or if } \boundarypiece \in \Sigma_\setminussign, \\
		%\boldsymbol g - \tensorsigma(\boldsymbol u^{k_\boundarypiece})\mathbf{n} & \text{if } \boundarypiece \in \Sigma_\setminussign \\
		- \Big(\boldsymbol g_0 + \tensorsigma(\boldsymbol u_\mathrm d) {\mathbf{n}}^{k_\boundarypiece}\Big) & \text{if } \boundarypiece \in \Sigma_{0,\mathrm p}.
	\end{cases}
\end{equation}
In other words, and as for Poisson's equation, $\boldsymbol d_\boundarypiece$ represents the Neumann error on the boundaries $\gamma_\mathrm n$ and $\gamma_\setminussign$ due to the defeaturing process, and the jump of the normal derivative of the defeatured solution on the boundaries $\gamma_{0,\mathrm p}$.
Moreover, recalling that the Lam\'e coefficients $\mu$ and $\lambda$ verify the well-possedness conditions~\eqref{eq:assumptionslame}, let
$\rho\geq 0$ come from the coercivity constant of the bilinear form $\mathfrak a(\boldsymbol{\cdot},\boldsymbol{\cdot})$ corresponding to problem~\eqref{eq:weakfeaturepblinelast}, explicitly defined by
\begin{equation}\label{eq:defrho}
	\rho := \begin{cases}
		\mu_\mathrm{min}                                       & \text{ if } \lambda \geq 0 \text{ a.e.,} \\
		\min(\mu_\mathrm{min}, \frac{3}{2}\kappa_\mathrm{min}) & \text{ otherwise.}
	\end{cases}
\end{equation}
Then, we define the \textit{a posteriori} defeaturing error estimator as:
\begin{equation}\label{eq:multiestimatorlinelast}
	\mathscr{E}(\boldsymbol u_\mathrm d) := \left(\sum_{\boundarypiece\in\Sigma} \mathscr{E}_\boundarypiece(\boldsymbol{u}_\mathrm d)^2 \right)^\frac{1}{2},
\end{equation}
where for all $\boundarypiece\in\Sigma$,
\begin{equation*}
	\mathscr{E}_\boundarypiece(\boldsymbol u_\mathrm d) := \rho^{-\frac{1}{2}}\left(|\boundarypiece|^\frac{1}{n-1} \left\|\boldsymbol d_\boundarypiece - \overline{\boldsymbol d_\boundarypiece}^\boundarypiece\right\|_{0,\boundarypiece}^2 + c_\boundarypiece^2 |\boundarypiece|^\frac{n}{n-1} \left\|\overline{\boldsymbol d_\boundarypiece}^\boundarypiece\right\|_{\ell^2}^2\right)^\frac{1}{2},
\end{equation*}
where $c_\boundarypiece$ is defined in~\eqref{eqp1:negconstant}, $\overline{\boldsymbol d_\boundarypiece}^\boundarypiece$ denotes the dimension-wise average value of $\boldsymbol d_\boundarypiece$ over $\boundarypiece$, and $\|\boldsymbol\cdot\|_{\ell^2}$ denotes the discrete $\ell^2$-norm as $\overline{\boldsymbol d_\boundarypiece}^\boundarypiece\in\mathbb R^n$.
Note that, similarly as in~\eqref{eq:estforeachfeatpoisson}, we can rewrite the estimator feature-wise as follows:
\begin{equation}\label{eq:estforeachfeatlinelast}
	\mathscr{E}(\boldsymbol u_\mathrm d) = \left(\sum_{k=1}^{N_f} \sum_{\boundarypiece\in\Sigma^k} \mathscr{E}_{\boundarypiece}(\boldsymbol{u}_\mathrm d)^2 \right)^\frac{1}{2} = \left(\sum_{k=1}^{N_f} \mathscr{E}^{k}(\boldsymbol u_\mathrm d)^2\right)^\frac{1}{2},
\end{equation}
where for all $k=1,\ldots,N_f$, we define $\mathscr{E}^{k}(\boldsymbol u_k)$ as the defeaturing error estimator for feature $F^k$, that is,
\begin{equation*}
	\mathscr{E}^k(\boldsymbol u_\mathrm d) := \left(\sum_{\boundarypiece\in\Sigma^k} \mathscr{E}_{\boundarypiece}(\boldsymbol{u}_\mathrm d)^2 \right)^\frac{1}{2}.
\end{equation*}
% Similarly as in~\eqref{eq:estforeachfeatpoisson}, the estimator can be computed feature-wise by evaluating the contributions of all boundaries $\boundarypiece\in\Sigma^k$ associated to every feature $k$.

The proposed estimator indicates that all the information on the error introduced by defeaturing, in the energy norm, is encoded in the boundary of the features, and can be accounted by suitably evaluating the error made on the normal traction of the solution.

\begin{remark} \label{rmk:compatcondmultilinelast}
	As in Remark~\ref{rmk:compatcondmultipoisson}, the terms involving the component-wise average values of $\boldsymbol d_\boundarypiece$ in the estimator $\mathscr E(\boldsymbol u_\mathrm d)$ only depend on the defeatured problem data. As a consequence, if these terms dominate, this means that the defeatured problem data should be more accurately chosen. Moreover, under the following reasonable vectorial data compatibility conditions~\eqref{eq:compatcondmultilinelast} and~\eqref{eq:compatcondmultilinelast2} for all $k=1,\ldots,N_f$, the defeaturing error estimator~\eqref{eq:multiestimatorlinelast} rewrites
	$$\mathscr E(\boldsymbol u_\mathrm d) := \rho^{-\frac{1}{2}}\left( \displaystyle\sum_{\boundarypiece\in\Sigma} \left|\boundarypiece\right|^{\frac{1}{n-1}} \left\| \boldsymbol d_\boundarypiece \right\|^2_{0,\boundarypiece}\right)^\frac{1}{2}.$$
\end{remark}

\begin{remark} \label{rmk:estmultitildelinelast}
	In a similar fashion as Remark~\ref{rmk:estmultitildepoisson}, note that
	\begin{align*}
		\mathscr{E}(\boldsymbol u_\mathrm d) \lesssim \rho^{-\frac{1}{2}} \left( \displaystyle\sum_{\boundarypiece\in\Sigma} c_\boundarypiece^2 \left|\boundarypiece\right|^{\frac{1}{n-1}} \left\| \boldsymbol d_\boundarypiece \right\|^2_{0,\boundarypiece}\right)^\frac{1}{2} =: \tilde{\mathscr{E}}(\boldsymbol u_\mathrm d).
	\end{align*}
	However, when $n=2$, and under the data compatibility conditions~\eqref{eq:compatcondmultilinelast} and~\eqref{eq:compatcondmultilinelast2}, $\tilde{\mathscr{E}}(\boldsymbol u_\mathrm d)$ is sub-optimal since in this case, $\tilde{\mathscr{E}}(\boldsymbol u_\mathrm d) \lesssim \displaystyle\max_{\boundarypiece\in\Sigma}\left( c_{\boundarypiece} \right) {\mathscr{E}}(\boldsymbol u_\mathrm d)$.
\end{remark}

==> stokes.tex <==
Finally, in this section, we consider the Stokes' equations and we define precisely the exact $\mathcal P(\Omega)$, defeatured $\mathcal P(\Omega_0)$, and extension problems $\mathcal P\big(\tilde F_\mathrm p^k\big)$ for all $k=1,\ldots,N_f$. Then in this context, we give a precise definition of the proposed reliable and efficient \textit{a posteriori} estimator $\mathscr E(\boldsymbol u_\mathrm d, p_\mathrm d)$ of the energy norm of the defeaturing error $\vertiii{ \left(\boldsymbol u - \boldsymbol u_\mathrm d, p-p_\mathrm d\right)}_\Omega$.

\subsection{Exact and defeatured problems}
Let us first introduce the Stokes problem $\mathcal P(\Omega)$ in the exact geometry $\Omega$. To do so, considering a function $\boldsymbol v:\Omega\to\mathbb R^n$, let $\tensorepsilon(\boldsymbol v)$ denote the linearized strain rate tensor in $\Omega$,
analogous to~\eqref{eq:linearizestrain}, and let $\tensorsigma(\boldsymbol v)$ be the viscous stress tensor of the considered fluid. Assuming the fluid to be Newtonian, Galilean invariance implies that
\begin{equation} \label{eq:constitutiverelationstokes1}
	\tensorsigma(\boldsymbol v) = 2\mu\,\tensorepsilon(\boldsymbol v) + \lambda (\boldsymbol \nabla \cdot \boldsymbol v)\pmb{\mathbb I}_n,
\end{equation}
where, in this case,  the constants $\mu > 0$ and $\lambda \geq 0$ are now the dynamic and bulk viscosities, respectively.
Assumption~\ref{asid:lame_constant} also applies in this case.
Note that in this section, $\tensorsigma(\boldsymbol v)$ is the viscous stress tensor and not the total Cauchy stress tensor that would be defined by
$\hat{\tensorsigma}(\boldsymbol v, q) := \tensorsigma(\boldsymbol{v}) - q\,\pmb{\mathbb I}_n$
for some function $q:\Omega\to\mathbb R$ in the space of pressures.

Now, let $\boldsymbol g_D\in \boldsymbol H^{\frac{3}{2}}(\Gamma_D)$, $\boldsymbol g\in \boldsymbol H^{\frac{1}{2}}(\Gamma_N)$, $f_c\in L^2(\Omega)$, and $\boldsymbol f\in \boldsymbol L^2\left(\Omega\right)$. We are interested in the following Stokes problem defined in the exact geometry $\Omega$: find $(\boldsymbol u, p)\in\boldsymbol H^{1}(\Omega)\times L^2(\Omega)$, the weak solution of
\begin{align}
	\mathcal P(\Omega): \quad
	\begin{cases}
		-\boldsymbol \nabla \cdot \tensorsigma (\boldsymbol u) + \nabla p =\boldsymbol f & \text{ in } \Omega    \\
		\boldsymbol \nabla \cdot \boldsymbol u = f_c                                     & \text{ in } \Omega    \\
		\boldsymbol u = \boldsymbol g_D                                                  & \text{ on } \Gamma_D  \\
		\tensorsigma (\boldsymbol u)\mathbf{n} - p\mathbf n= \boldsymbol g               & \text{ on } \Gamma_N,
	\end{cases}\label{eqid:originalstokespb}
\end{align}
that is, $(\boldsymbol u,p) \in \boldsymbol H^1_{\boldsymbol g_D, \Gamma_D}(\Omega)\times L^2(\Omega)$ satisfies for all $(\boldsymbol v,q)\in \boldsymbol H^1_{\boldsymbol 0,\Gamma_D}(\Omega)\times L^2(\Omega)$,
\begin{equation}
	\begin{aligned}
		\mathfrak a(\boldsymbol{u}, \boldsymbol{v}) + \mathfrak b(p,\boldsymbol{v}) & = \int_\Omega \boldsymbol f \cdot \boldsymbol v \,\mathrm dx + \int_{\Gamma_N} \boldsymbol g \cdot \boldsymbol v \,\mathrm ds, \\
		\mathfrak b(q,\boldsymbol{u})                                               & = -\int_{\Omega} q f_c\,\mathrm dx.\label{eqid:weakoriginalstokespb}
	\end{aligned}
\end{equation}
where for all $\boldsymbol{v}, \boldsymbol{w}\in \boldsymbol{H}^1(\Omega)$ and all $q\in L^2(\Omega)$,
\begin{align}
	\mathfrak a(\boldsymbol{w}, \boldsymbol{v}) & := \displaystyle\int_\Omega \tensorsigma (\boldsymbol u) : \tensorepsilon(\boldsymbol v) \,\mathrm dx, \label{eq:defastokes} \\
	\mathfrak b(q,\boldsymbol{v})               & := - \int_\Omega p\boldsymbol \nabla \cdot \boldsymbol{v} \,\mathrm dx. \label{eq:defbstokes}
\end{align}
Note that if $f_c \equiv 0$, then~\eqref{eqid:originalstokespb} is also the system of equations describing the linear elastic problem of Section~\ref{s:linelast} in the incompressible limit $\lambda \to \infty$, and~\eqref{eq:constitutiverelationstokes1} simplifies to
\begin{equation}\label{eq:constitutiverelationstokes2}
	\boldsymbol \sigma(\boldsymbol v) = 2\mu \boldsymbol{\varepsilon}(v).
\end{equation}
Moreover, since
$$\nabla \cdot \big( \lambda (\nabla\cdot \boldsymbol v)\pmb{\mathbb I}_n\big) = \nabla(\lambda \nabla \cdot \boldsymbol v),$$
if we use the following change of variables,
\begin{equation}
	p' := p-\lambda \nabla u, \quad \boldsymbol{\sigma}'(\boldsymbol{u}) := 2\mu\boldsymbol{\varepsilon}(\boldsymbol{u}),
\end{equation}
then problem~\eqref{eqid:originalstokespb} remains identical if we replace $p$ by $p'$ and $\boldsymbol{\sigma}(\boldsymbol u)$ by $\boldsymbol{\sigma}'(\boldsymbol u)$. Therefore, in the following, we adopt this change of variables and we assume that $\boldsymbol{\sigma}(\boldsymbol u)$ is expressed as in~\eqref{eq:constitutiverelationstokes2} from now on.

If we equip $\boldsymbol H^1_{\boldsymbol 0, \Gamma_D}(\Omega)$ with the norm $\| \boldsymbol \nabla \boldsymbol \cdot \|_{0,\Omega}$, it is possible to show by Ladyzhenskaya-Babu\v{s}ka-Brezzi theorem~\cite{boffi2013mixed} that problem~\eqref{eqid:weakoriginalstokespb} is well-posed.
% However, note that this problem is never solved in practice, as it is assumed to be computationally too expensive. \\

Let us introduce the corresponding Stokes problem $\mathcal P(\Omega_0)$ in the defeatured geometry $\Omega_0$. To do so, we need to choose an $\boldsymbol L^2$-extension of $\boldsymbol f$ and an $L^2$-extension of $f_c$ in the negative components of the features $F_\mathrm n$, that we still write $\boldsymbol f$ and $f_c$ by abuse of notation. Moreover, we assume that the viscous stress tensor $\tensorsigma$ also satisfies~\eqref{eq:constitutiverelationstokes2} on functions defined everywhere in $\Omega_0$.
Then instead of the exact problem~\eqref{eqid:originalstokespb} and similarly to~\eqref{eqid:simplpblinelast}, the following defeatured problem is solved: after choosing $\boldsymbol g_0\in \boldsymbol H^{\frac{1}{2}}\left(\gamma_0\right)$, find the weak solution $(\boldsymbol u_0,p_0)\in \boldsymbol H^1(\Omega_0)\times L^2(\Omega_0)$ of
\begin{align} \label{eqid:simplstokespb}
	\mathcal P(\Omega_0): \quad \begin{cases}
		-\boldsymbol \nabla \cdot \tensorsigma (\boldsymbol u_0) + \nabla p_0 =\boldsymbol f & \text{ in } \Omega_0                 \\
		\boldsymbol \nabla \cdot \boldsymbol u_0 = f_c                                       & \text{ in } \Omega_0                 \\
		\boldsymbol u_0 = \boldsymbol g_D                                                    & \text{ on } \Gamma_D                 \\
		\tensorsigma (\boldsymbol u_0)\mathbf{n} - p_0\mathbf n = \boldsymbol g              & \text{ on } \Gamma_N\setminus \gamma \\
		\tensorsigma (\boldsymbol u_0)\mathbf{n}_0 - p_0\mathbf n = \boldsymbol g_0          & \text{ on } \gamma_0,
	\end{cases}
\end{align}
that is, $(\boldsymbol u_0,p_0)\in \boldsymbol H^1_{\boldsymbol g_D,\Gamma_D}(\Omega_0)\times L^2(\Omega_0)$ satisfies for all $(\boldsymbol v_0,q_0)\in \boldsymbol H^1_{\boldsymbol 0,\Gamma_D}(\Omega_0)\times L^2(\Omega_0)$,
\begin{align}
	\int_{\Omega_0} \tensorsigma (\boldsymbol u_0) : \tensorepsilon(\boldsymbol v_0) \,\mathrm dx - \int_\Omega p_0\boldsymbol \nabla \cdot \boldsymbol{v}_0 \,\mathrm dx & = \int_{\Omega_0} \boldsymbol f \cdot \boldsymbol v_0 \,\mathrm dx + \int_{\Gamma_N\setminus \gamma} \boldsymbol g \cdot \boldsymbol v_0 \,\mathrm ds + \int_{\gamma_0} \boldsymbol g_0 \cdot \boldsymbol v_0 \,\mathrm ds,\nonumber \\
	-\displaystyle\int_\Omega q_0\boldsymbol \nabla \cdot \boldsymbol{u}_0 \,\mathrm dx                                                                                   & = -\int_{\Omega} q_0 f_c\,\mathrm dx. \label{eq:weaksimplstokespb}
\end{align}
By Ladyzhenskaya-Babu\v{s}ka-Brezzi theorem, problem~\eqref{eq:weaksimplstokespb} is well-posed. As for the Poisson and linear elasticity problems, the choice of the defeatured problem data $\boldsymbol f$ and $f_c$ in $F_\mathrm n^k$ for $k=1,\ldots,N_f$ and $\boldsymbol g_0$ on $\gamma_0$ will be guided by Remark~\ref{rmk:compatcondmultistokes}. As for Poisson and linear elasticity problems, the best possible choices satisfy a conservation assumption of the solution flux in the positive and negative components of the features given by~\eqref{eq:compatcondmultilinelast} for all $k=1,\ldots,N_f$.

Now, for all $k=1,\ldots,N_f$, we need to extend the solution $(\boldsymbol u_0, p_0)$ of~\eqref{eq:weaksimplstokespb} to $\tilde F^k_\mathrm p$ as discussed in Section~\ref{ss:pbpres}, where $\tilde F^k_\mathrm p$ satisfies the properties given in~\eqref{eq:condextension}. To do so, let us choose an $\boldsymbol L^2$-extension of the restriction $\boldsymbol f\vert_{F_\mathrm p^{k}}$ and an $L^2$-extension of the restriction $f_c\vert_{F_\mathrm p^{k}}$ in $G_\mathrm p^k := \tilde F_\mathrm p^k \setminus \overline{F_\mathrm p^k}$, that we still write $\boldsymbol f$ and $f_c$ by abuse of notation. Moreover, we assume that the viscous stress tensor $\tensorsigma$ also satisfies~\eqref{eq:constitutiverelationstokes2} on functions defined in $\tilde F_\mathrm p^k$. Then, similarly to~\eqref{eq:featurepblinelast}, we define for all $k=1,\ldots,N_f$ the following extension of the solution $(\boldsymbol u_0, p_0)$ of \eqref{eqid:simplstokespb} in $\tilde F^k_\mathrm p$:
after choosing $\tilde{\boldsymbol g}^k\in \boldsymbol H^\frac{1}{2}(\tilde \gamma^k)$, find $(\boldsymbol u_k, p_k)\in \boldsymbol H^1\left(\tilde F_\mathrm p^k\right)\times L^2\left(\tilde F_\mathrm p^k\right)$, the weak solution of
\begin{align} \label{eq:featurestokespb}
	\mathcal P\Big(\tilde F_\mathrm p^k\Big): \quad \begin{cases}
		-\boldsymbol \nabla \cdot \tensorsigma (\boldsymbol u_k) + \nabla p_k =\boldsymbol f                    & \text{ in } \tilde{F}_\mathrm p^k  \\
		\boldsymbol \nabla \cdot \boldsymbol u_k = f_c                                                          & \text{ in } \tilde{F}_\mathrm p^k  \\
		\boldsymbol u_k = \boldsymbol u_0                                                                       & \text{ on } \gamma_{0,\mathrm p}^k \\
		\tensorsigma (\boldsymbol u_k)\tilde{\mathbf{n}}^k - p_k \tilde{\mathbf{n}}^k = \tilde{\boldsymbol g}^k & \text{ on } \tilde \gamma^k        \\
		\tensorsigma (\boldsymbol u_k)\tilde{\mathbf{n}}^k - p_k \tilde{\mathbf{n}}^k = \boldsymbol g           & \text{ on } \gamma_\intersign^k,
	\end{cases}
\end{align}
that is, $(\boldsymbol u_k, p_k)\in \boldsymbol H^1_{\boldsymbol u_0,\gamma_{0,\mathrm p}^k}\left(\tilde F_\mathrm p^k\right)\times L^2\left(\tilde F_\mathrm p^k\right)$
satisfies for all $(\boldsymbol v^k,q^k)\in \boldsymbol H^1_{\boldsymbol 0,\gamma_{0,\mathrm p}^k}\left(\tilde{F}_\mathrm p^k\right)\times L^2\left(\tilde F_\mathrm p^k\right)$,
\begin{align}
	\int_{\tilde{F}_\mathrm p^k} \tensorsigma (\boldsymbol u_k) : \tensorepsilon(\boldsymbol v^k) \,\mathrm dx -\displaystyle\int_{\tilde{F}_\mathrm p^k} p_k\boldsymbol \nabla \cdot \boldsymbol{v}^k \,\mathrm dx & = \int_{\tilde{F}_\mathrm p^k} \boldsymbol f \cdot \boldsymbol v^k \,\mathrm dx + \int_{\tilde \gamma^k} \tilde{\boldsymbol g}^k \cdot \boldsymbol v^k \,\mathrm ds + \int_{\gamma_\intersign^k} \boldsymbol g \cdot \boldsymbol v^k \,\mathrm ds, \nonumber \\
	-\displaystyle\int_{\tilde{F}_\mathrm p^k} q^k\boldsymbol \nabla \cdot \boldsymbol{u}_k \,\mathrm dx                                                                                                            & = -\int_{\tilde{F}_\mathrm p^k} q^k f_c\,\mathrm dx. \label{eq:weakfeaturestokespb}
\end{align}
By Ladyzhenskaya-Babu\v{s}ka-Brezzi theorem, problem~\eqref{eq:weakfeaturestokespb} is well-posed. The choice of the defeatured problem data $\boldsymbol f$ and $f_c$ in $G_\mathrm p^k$, and $\tilde{\boldsymbol g}^k$ on $\tilde \gamma^k$ for $k=1,\ldots,N_f$ will be guided by Remark~\ref{rmk:compatcondmultistokes}. We anticipate here that as before, the best possible choices satisfy a conservation assumption of the solution flux in every feature's extension $G_\mathrm p^k$, given by~\eqref{eq:compatcondmultilinelast2}.

Then, the defeatured solution $(\boldsymbol u_\mathrm d,p_\mathrm d) \in \boldsymbol H_{\boldsymbol g_D,\Gamma_D}(\Omega)\times L^2(\Omega)$ is defined from $(\boldsymbol u_0, p_0)$ and $(\boldsymbol u_k, p_k)$ for $k=1,\ldots,N_f$ as in~\eqref{eqid:defudmulti} and we define the defeaturing error as
\begin{equation}\label{eq:defeaterrorstokes}
	\vertiii{ \left(\boldsymbol u - \boldsymbol u_\mathrm d, p-p_\mathrm d\right)}_\Omega = \left(\int_\Omega \tensorsigma(\boldsymbol u-\boldsymbol u_\mathrm d) : \tensorepsilon(\boldsymbol u-\boldsymbol u_\mathrm d) \,\mathrm dx\right)^\frac{1}{2} + \mu^{-\frac{1}{2}} \|p-p_\mathrm d\|_{0,\Omega}.
\end{equation}

\subsection{Defeaturing error estimator}
Let us recall the definition of the defeatured solution $(\boldsymbol u_\mathrm d, p_\mathrm d)$ from~\eqref{eqid:defudmulti}, and the definitions of $\Sigma$, $\Sigma^k$, $\Sigma_\mathrm n$, $\Sigma_{0,\mathrm p}$, and $\Sigma_\setminussign$ from~\eqref{eq:sigmamulti}. Then, let $k_\boundarypiece \equiv k$ if $\boundarypiece \in \Sigma^k$ for some $k=1,\ldots,N_f$, and let us redefine $\boldsymbol d_\boundarypiece$ for all $\boundarypiece \in \Sigma$ in the context of Stokes equations. That is, let
\begin{equation} \label{eq:dsigmastokes}
	\boldsymbol d_\boundarypiece \equiv \begin{cases}\vspace{1mm}
		\boldsymbol g - \tensorsigma(\boldsymbol u_\mathrm d)\mathbf{n} + p_\mathrm d\mathbf{n}                                                         & \text{if } \boundarypiece \in \Sigma_\mathrm n \text{ of if } \boundarypiece\in \Sigma_\setminussign, \\
		%\boldsymbol g - \tensorsigma (\boldsymbol u^{k_\boundarypiece})\mathbf{n} + p^{k_\boundarypiece}\mathbf{n} & \text{if } \boundarypiece \in \Sigma_\setminussign \\
		-\Big(\boldsymbol g_0 + \tensorsigma (\boldsymbol u_\mathrm d){\mathbf{n}}^{k_\boundarypiece} - p_\mathrm d{\mathbf{n}}^{k_\boundarypiece}\Big) & \text{if } \boundarypiece \in \Sigma_{0,\mathrm p}.
	\end{cases}
\end{equation}
In other words, and as for Poisson's and linear elasticity equations, $\boldsymbol d_\boundarypiece$ represents the Neumann error on the boundaries $\gamma_\mathrm n$ and $\gamma_\setminussign$ due to the defeaturing process, and the jump of the normal derivative of the defeatured solution on the boundaries $\gamma_{0,\mathrm p}$.
Then, we define the \textit{a posteriori} defeaturing error estimator as:
\begin{equation}\label{eq:multiestimatorstokes}
	\mathscr{E}(\boldsymbol u_\mathrm d, p_\mathrm d) := \left(\sum_{\boundarypiece\in\Sigma} \mathscr{E}_\boundarypiece(\boldsymbol{u}_\mathrm d, p_\mathrm d)^2 \right)^\frac{1}{2},
\end{equation}
where for all $\boundarypiece\in\Sigma$,
\begin{equation*}
	\mathscr{E}_\boundarypiece(\boldsymbol u_\mathrm d, p_\mathrm d) := 3\mu^{-\frac{1}{2}}\left(|\boundarypiece|^\frac{1}{n-1} \left\|\boldsymbol d_\boundarypiece - \overline{\boldsymbol d_\boundarypiece}^\boundarypiece\right\|_{0,\boundarypiece}^2 + c_\boundarypiece^2 |\boundarypiece|^\frac{n}{n-1} \left\|\overline{\boldsymbol d_\boundarypiece}^\boundarypiece\right\|_{\ell^2}^2\right)^\frac{1}{2},
\end{equation*}
where $c_\boundarypiece$ is defined in \eqref{eqp1:negconstant}, $\overline{\boldsymbol d_\boundarypiece}^\boundarypiece$ denotes the dimension-wise average value of $\boldsymbol d_\boundarypiece$ over $\boundarypiece$, and $\|\boldsymbol\cdot\|_{\ell^2}$ denotes the discrete $\ell^2$-norm as $\overline{\boldsymbol d_\boundarypiece}^\boundarypiece\in\mathbb R^n$.
Note that, as for the Poisson's and linear elasticity problems, we can rewrite the estimator feature-wise as
% in~\eqref{eq:estforeachfeatpoisson}, just accumulating the contributions of all boundaries $\boundarypiece\in\Sigma^k$ associated to every feature $k$.
\begin{equation}\label{eq:estforeachfeatstokes}
	\mathscr{E}(\boldsymbol u_\mathrm d, p_\mathrm d) = \left(\sum_{k=1}^{N_f} \sum_{\boundarypiece\in\Sigma^k} \mathscr{E}_{\boundarypiece}(\boldsymbol{u}_\mathrm d, p_\mathrm d)^2 \right)^\frac{1}{2} = \left(\sum_{k=1}^{N_f} \mathscr{E}^{k}(\boldsymbol u_\mathrm d, p_\mathrm d)^2\right)^\frac{1}{2},
\end{equation}
where for all $k=1,\ldots,N_f$, we define $\mathscr{E}^{k}(\boldsymbol u_k, p_k)$ as the defeaturing error estimator for feature $F^k$, that is,
\begin{equation*}
	\mathscr{E}^k(\boldsymbol u_\mathrm d, p_\mathrm d) := \left(\sum_{\boundarypiece\in\Sigma^k} \mathscr{E}_{\boundarypiece}(\boldsymbol{u}_\mathrm d, p_\mathrm d)^2 \right)^\frac{1}{2}.
\end{equation*}

The proposed estimator indicates that all the information on the error introduced by defeaturing is encoded in the boundary of the features, and can be accounted by suitably evaluating the error made on the normal viscous stress and pressure of the solution.

\begin{remark} \label{rmk:compatcondmultistokes}
	Similarly to Remarks~\ref{rmk:compatcondmultipoisson} and~\ref{rmk:compatcondmultilinelast}, the terms involving the component-wise average values of $\boldsymbol d_\boundarypiece$ in $\mathscr E(\boldsymbol u_\mathrm d, p_\mathrm d)$ only depend on the defeatured problem data. As a consequence, if these terms dominate, this means that the defeatured problem data should be more accurately chosen. Moreover, under the reasonable data compatibility conditions~\eqref{eq:compatcondmultilinelast} and~\eqref{eq:compatcondmultilinelast2} that represent flux conservation assumptions in this context, the defeaturing error estimator~\eqref{eq:multiestimatorstokes} rewrites
	$\mathscr E(\boldsymbol u_\mathrm d, p_\mathrm d) := \mu^{-\frac{1}{2}}\left( \displaystyle\sum_{\boundarypiece\in\Sigma} \left|\boundarypiece\right|^{\frac{1}{n-1}} \left\| \boldsymbol d_\boundarypiece \right\|^2_{0,\boundarypiece}\right)^\frac{1}{2}.$
\end{remark}

\begin{remark} \label{rmk:estmultitildestokes}
	Similarly to Remark~\ref{rmk:estmultitildepoisson} and~\ref{rmk:estmultitildelinelast}, note that
	\begin{align*}
		\mathscr{E}(\boldsymbol u_\mathrm d, p_\mathrm d) \lesssim \mu^{-\frac{1}{2}}\left( \displaystyle\sum_{\boundarypiece\in\Sigma} c_\boundarypiece^2 \left|\boundarypiece\right|^{\frac{1}{n-1}} \left\| \boldsymbol d_\boundarypiece \right\|^2_{0,\boundarypiece}\right)^\frac{1}{2} =: \tilde{\mathscr{E}}(\boldsymbol u_\mathrm d, p_\mathrm d).
	\end{align*}
	However, when $n=2$ and under the flux conservation conditions~\eqref{eq:compatcondmultilinelast} and~\eqref{eq:compatcondmultilinelast2}, $\tilde{\mathscr{E}}(\boldsymbol u_\mathrm d, p_\mathrm d)$ is sub-optimal since in this case, $\tilde{\mathscr{E}}(\boldsymbol u_\mathrm d, p_\mathrm d) \lesssim \displaystyle\max_{\boundarypiece\in\Sigma}\left( c_{\boundarypiece} \right) {\mathscr{E}}(\boldsymbol u_\mathrm d, p_\mathrm d)$.
\end{remark}


